DevOps Adoption: Eight Emergent Perspectives

DevOps is an approach based on lean and agile principles in which business, development, operations, and quality teams cooperate to deliver software continuously aiming at reducing time to market, and receiving constant feedback from customers. However, implementing DevOps can be a complex and challenging mission due it requires significant paradigm shift. Consequently, many failures and misconceptions can occur about DevOps adoption by organizations, despite its numerous benefits. This work identifies, describes, and compares different perspectives related to DevOps adoption in academy and industry. The perspectives can be understood as factors or variables that influence or help to understand the DevOps journey. We employed a sequential multi-method research approach, including Systematic Literature Review (SLR) and Case Study. As a result, eight perspectives were found: concepts, models, principles, practices, difficulties, challenges, benefits, and strategies. More specifically, the SLR produced 390 items, which can be understood as occurrences of a perspective. The conducted case study confirmed 75 items, corroborating the SLR findings, while another 29 items emerged. This global view on DevOps adoption may guide beginners, both theorists, and practitioners, to make the necessary organizational transformation less painful.

==> body/footer/authors-biography.tex <==
\begin{IEEEbiography}{First A. Author}{\,}current employment (is
currently with XYZ Corporation, New York, NY, USA). Author's latest degree received or which he/she is currently pursuing (He received the B.S. degree and the M.S. degree...."). Author's research interest. Association with any official journals or conferences; major professional and/or academic achievements, i.e., best paper awards, research grants, etc.; any publication information (number of papers and titles of books published). Author membership information, e.g., is a member of the IEEE and the IEEE Computer Society, if applicable, is noted at the end of the biography. Biography is limited to single paragraph only (He is a member of IEEE, etc.). All biographies should be limited to one paragraph, five to six sentences, consisting of the following: (e.g., ``Dr. Author received a B.S. degree and an M.S. degree $\ldots$.''), including years achieved; association with any official journals or conferences; major professional and/or academic achievements, i.e., best paper awards, research grants, etc.; any publication information (number of papers and titles of books published); current research interests; association with any professional associations. Author membership information, e.g., is a member of the IEEE and the IEEE Computer Society, if applicable, is noted at the end of the biography. Contact him/her at faauthor@xyz.com.
\end{IEEEbiography}

\begin{IEEEbiography}{Second B. Author, Jr.,}{\,}is with ABC Corporation, Bblingen, Germany. Ms. Author's biography appears here.  Contact him/her at sbauthor@abc.com.
\end{IEEEbiography}

\begin{IEEEbiography}{Third C. Author, III,}{\,}is with DEF Corporation, Tokyo, Japan. Dr. Author's biography appears here.  Contact him/her at tcauthor@def.com.
\end{IEEEbiography}

==> body/header/authors-ieee-template.tex <==

\author{\textsuperscript{1}Mauro Lourenço Pedra}
\affil{Graduate Program in Informatics, Federal University of Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil - mauro.pedra@ufrj.br - https://orcid.org/0000-0003-2802-6440}

\author{\textsuperscript{1}Mônica Ferreira da Silva}
\affil{Graduate Program in Informatics, Federal University of Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil - monica.silva@ppgi.ufrj.br -  https://orcid.org/0000-0003-0951-6612}

\author{\textsuperscript{2}Leonardo Guerreiro Azevedo}
\affil{IBM Research, Rio de Janeiro, Brazil - lga@br.ibm.com -- https://orcid.org/0000-0002-2109-1285}



% \author{Mônica Ferreira da Silva}
% \affil{Graduate Program in Informatics, Federal University of Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil }

% \author{T. C. Author, III}
% \affil{Third Affiliation}


% \author{\IEEEauthorblockN{Mauro Lourenço Pedra}
% \IEEEauthorblockA{\textit{Graduate Program in Informatics} \\
% \textit{Federal University of Rio de Janeiro}\\
% Rio de Janeiro, RJ, Brazil \\
% mauro.pedra@ufrj.br}
% \and
% \IEEEauthorblockN{Mônica Ferreira da Silva}
% \IEEEauthorblockA{\textit{Graduate Program in Informatics} \\
% \textit{Federal University of Rio de Janeiro}\\
% Rio de Janeiro, RJ, Brazil \\
% https://orcid.org/0000-0003-0951-6612}
% \and
% \IEEEauthorblockN{Leonardo Guerreiro Azevedo}
% \IEEEauthorblockA{\textit{IBM Research}\\
% Rio de Janeiro, RJ, Brazil \\
% lga@br.ibm.com}
% }


% \title{Title: No More Than Four Lines}





==> body/header/department.tex <==
\sptitle{Department: Head}
\editor{Editor: Name, xxxx@email}

==> body/header/keywords-ieee-template.tex <==
\begin{IEEEkeywords}
Software Engineering, Agile,  \devops{} Adoption, \devops{} implementation, \devops{} Dimensions
\end{IEEEkeywords}

%DevOps, Adoption, Implementation, Dimensions
% perspectivas, DevOps, adoção, desenvolvimento, operações, software
%dimensions / perspectives, DevOps, Adoption, Development, Operations, Software

